ArtisanGS: Interactive Tools for Gaussian Splat Selection with AI and Human in the Loop

Representation in the family of 3D Gaussian Splats (3DGS) are growing into a viable alternative to traditional graphics for an expanding number of application, including recent techniques that facilitate physics simulation and animation. However, extracting usable objects from in-the-wild captures remains challenging and controllable editing techniques for this representation are limited. Unlike the bulk of emerging techniques, focused on automatic solutions or high-level editing, we introduce an interactive suite of tools centered around versatile Gaussian Splat selection and segmentation. We propose a fast AI-driven method to propagate user-guided 2D selection masks to 3DGS selections. This technique allows for user intervention in the case of errors and is further coupled with flexible manual selection and segmentation tools. These allow a user to achieve virtually any binary segmentation of an unstructured 3DGS scene. We evaluate our toolset against the state-of-the-art for Gaussian Splat selection and demonstrate their utility for downstream applications by developing a user-guided local editing approach, leveraging a custom Video Diffusion Model. With flexible selection tools, users have direct control over the areas that the AI can modify. Our selection and editing tools can be used for any in-the-wild capture without additional optimization.

==> fig/fig_completion.tex <==
\begin{figure*}[ht!]
	\centering
	\subfloat[User-guided object completion]{%
		\includegraphics[width=0.63\linewidth]{img/completion.png}}
        \hfill
	\subfloat[Video model block]{%
		\includegraphics[width=0.26\linewidth]{img/video_block.png}}
	\caption{\textbf{Object completion}(\S\ref{sec:refine}): after the user marks region to be completed and iterates on a 2D inpainting for one view, we apply a custom video inpainting model to propagate the result to multi-view consistent frames, which are used to fine-tune the 3DGS object.}
    % (a); our video diffusion block is shown in b.}
	\label{fig:segment_manual}
\end{figure*}

==> fig/fig_nvos_bad_scribbles.tex <==
\begin{figure}
\centering
    \hfill
    \subfloat[NVOS scribbles]{%
    \includegraphics[width=0.19\linewidth]{img/nvos/orchids_scribbles.png}}
    \subfloat[NVOS ground truth mask]{%
    \includegraphics[width=0.19\linewidth]{img/nvos/issue_gt_mask_nvos.png}}
    \subfloat[Our points inputs]{%
    \includegraphics[width=0.19\linewidth]{img/nvos/viz_summary.png}}
    \subfloat[SAM 
 mask from our points inputs]{%
    \includegraphics[width=0.19\linewidth]{img/nvos/mask_and_queries_3.png}}
    \hfill
    \caption{NVOS scribbles are not complete, the scribbles on the left is not covering the ground truth mask in the yellow box. Our inputs are very simples and lead to good masks output by SAM}
    \label{fig:nvos_bad_scribbles}
\end{figure}

==> fig/fig_nvos_inputs.tex <==
\begin{figure}
\centering
            \hfill
		\includegraphics[width=0.19\linewidth]{img/nvos/mask_and_queries_0.png}
		\includegraphics[width=0.19\linewidth]{img/nvos/mask_and_queries_1.png}
		\includegraphics[width=0.19\linewidth]{img/nvos/mask_and_queries_2.png}
		\includegraphics[width=0.19\linewidth]{img/nvos/mask_and_queries_3.png}
		\includegraphics[width=0.19\linewidth]{img/nvos/mask_and_queries_4.png}
            \hfill
	\caption{Our segmentation process for the input of SAM. Green points are positive clicks, red points are negative clicks}
	\label{fig:segment_clicks}
\end{figure}

==> fig/tb_inpaint_reconstruct.tex <==
\begin{table}[t!]
\centering

\begingroup
\footnotesize{
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\begin{tabular}{@{}|l||lll|lll|@{}}
\Xhline{2.0pt}
& \multicolumn{3}{c|}{GSO} & \multicolumn{3}{c|}{Toys5}\\ 
\textbf{Method} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} \\
& (unmasked) & & & (unmasked) & & \\
\Xhline{2.0pt}
MVInpainter & & & & & & \\
Wonder3D & & & & & & \\
Infusion & & & & & & \\
\Xhline{2.0pt}
Ours (no plucker) & & & & & &\\
Ours (no epipolar) & & & & & &\\
Ours (full model) & & & & & & \\
\Xhline{2.0pt}
\end{tabular}
}
\endgroup
\caption{We evaluate our method on the full task of 3D object inpainting against three baselines on 100 samples from the GSO dataset.}
\label{tb:inp_model_eval}
\end{table}

==> text/sec_conclusion.tex <==
\section{Conclusion}
